Large-scale self-assembled nanophotonic scintillators for X-ray imaging

Scintillators are essential for converting X-ray energy into visible light in imaging technologies. Their widespread application in imaging technologies has been enabled by scalable, high-quality, and affordable manufacturing methods. Nanophotonic scintillators, which feature nanostructures at the scale of their emission wavelength, provide a promising approach to enhance emission properties like light yield, decay time, and directionality. However, scalable fabrication of such nanostructured scintillators has been a significant challenge, impeding their widespread adoption. Here, we present a scalable fabrication method for large-area nanophotonic scintillators based on the self-assembly of chalcogenide glass photonic crystals. This technique enables the production of nanophotonic scintillators over wafer-scale areas, achieving a six-fold enhancement in light yield compared to unpatterned scintillators. We demonstrate this approach using a conventional X-ray scintillator material, cerium-doped yttrium aluminum garnet (YAG:Ce). By analyzing the influence of surface nanofabrication disorder, we establish its effect on imaging performance and provide a route towards large-scale scintillation enhancements without decrease in spatial resolution. Finally, we demonstrate the practical applicability of our nanophotonic scintillators through X-ray imaging of biological and inorganic specimens. Our results indicate that this scalable fabrication technique could enable the industrial implementation of a new generation of nanophotonic-enhanced scintillators, with significant implications for advancements in medical imaging, security screening, and nondestructive testing.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
